Representation Learning Beyond Linear Prediction Functions

Recent papers on the theory of representation learning has shown the importance of a quantity called diversity when generalizing from a set of source tasks to a target task. Most of these papers assume that the function mapping shared representations to predictions is linear, for both source and target tasks. In practice, researchers in deep learning use different numbers of extra layers following the pretrained model based on the difficulty of the new task. This motivates us to ask whether diversity can be achieved when source tasks and the target task use different prediction function spaces beyond linear functions. We show that diversity holds even if the target task uses a neural network with multiple layers, as long as source tasks use linear functions. If source tasks use nonlinear prediction functions, we provide a negative result by showing that depth-1 neural networks with ReLu activation function need exponentially many source tasks to achieve diversity. For a general function class, we find that eluder dimension gives a lower bound on the number of tasks required for diversity. Our theoretical results imply that simpler tasks generalize better. Though our theoretical results are shown for the global minimizer of empirical risks, their qualitative predictions still hold true for gradient-based optimization algorithms as verified by our simulations on deep neural networks.

==> Representation%20Learning%20(Version%2012650)/sec0_negative_result.tex <==
\section{Negative transfer when source tasks are more complex}
\label{sec:negative_res}
Before introducing the cases that allow transfer, we first look at a case where transfer is impossible. 

Let the source task use a linear mapping following the shared representation and the target task directly learns the representation. In other words, $f_{ta}^*$ is identical mapping and known to the learner. We further consider $\mathcal{F}_{so} = \{z \mapsto w^T z: w \in \mathbb{R}^p\}$ and $\mathcal{H} = \{x\mapsto Hx : H \in \mathbb{R}^{p \times d}\}$. The interesting case is when $p \ll d$. Let the optimal representation be $H^*$ and the true prediction function for each source task be $w^*_1, \dots, w^*_T$. In the best scenario, we assume that there is no noise in the source tasks and each source task collects as many samples as possible, such that we will have an accurate estimation on each $w_t^{*T}H^* \in \mathbb{R}^{p \times d}$ which we denote by $W_t^*$.

However, the hypothesis class given the information from source tasks are 
$$
    \{H \in \mathbb{R}^{p \times d}: \exists w \in \mathbb{R}^p,  w^TH = W_t \text{ for all } t = 1, \dots, T\}.
$$

As $H^*$ is in the above class, any $QH^*$ for some rotation matrix $Q \in \mathbb{R}^{p \times p}$ is also in the class. In other words, a non-reducible error of learnt representation is $\max_{ Q}\|H^* - QH^*\|_2^2$ in the worst case.

More generally, we give a condition for negative transfer. Consider a single source task $f_{so}^*$. Let $
    \mathcal{H}_{so}^* \coloneqq \argmin_{h \in \mathcal{H}} \min_{f\in \mathcal{F}_{so}} \mathcal{E}_{so}(f, h)
$ and $\mathcal{H}_{ta}^* \coloneqq \argmin_{h \in \mathcal{H}} \min_{f \in \mathcal{F}_{ta}} \mathcal{E}_{ta}(f, h)$. In fact, if one hopes to get a representation learning benefit with zero bias ($\mu = 0$), we need all $h \in \mathcal{H}_{so}^*$ to satisfy $\inf_{f \in \mathcal{F}_{ta}}\mathcal{E}_{ta}(f, h) = 0$, i.e. any representation that is optimal in the source task is optimal in the target task as well. Equivalently, we will need $\mathcal{H}_{so}^* \subset \mathcal{H}_{ta}^*$. As shown in Proposition \ref{prop:neg}, the definition of \textit{transferable} captures the case well.

\begin{prop}
\label{prop:neg}
If there exists a $h' \in \mathcal{H}^*_{so}$ such that $h' \notin \mathcal{H}_{ta}^*$, then $\min_{f_{ta}}\mathcal{E}_{ta}(f_{ta}, h') > 0$. Furthermore, there is no $\nu < \infty$, such that $f^*_{so}$ is $(\nu, 0)$-transferable to $f^*_{ta}$. %\ziping{Check the notations so that they are consistent.}
\end{prop}

\begin{proof}
The first statement is by definition. Plugging $g'$ into the Definition \ref{defn:transferable}, we will have $\nu = \infty$ 
\end{proof}

The negative transfer happens when the optimal representation for source tasks may not be optimal for the target task. As the case in our linear example, this is a result of more complex $\mathcal{F}_{so}$, which allows more flexibility to reduce errors. This inspires us to consider the opposite case where $\mathcal{F}_{ta}$ is more complex than $\mathcal{F}_{so}$.

==> Representation%20Learning%20(Version%2012650)/sec1_source_task_rep.tex <==
\section{Source task as a representation}
\label{sec:sour_repre}
Before discussing more general settings, we first consider a single source task, which we refer to $so$. Assume that the source task itself is a representation of the target task. Equivalently, the source task has a known prediction function $f^*_{so}(x) = x$. This is a commonly-used framework when we decompose a complex task into several simple tasks and use the output of simple tasks as the input of a higher-level task.

A widely-used transfer learning method, called offset learning, which assumes $f^*_{ta}(x) = f^*_{so}(x) + w^*_{ta}(x)$ for some offset function $w^*_{ta}$, also applies here. The offset method enjoys its benefits when $w_{ta}$ has low complexity and can be learnt with few samples. It is worth mentioning that our setting covers a more general setting in \cite{du2017hypothesis}, which assumes $f^*_{ta}(x) = G(f^*_{so}(x), w^*_{ta}(x))$ for some known transformation function $G$ and unknown $w_{ta}^*$.

\iffalse
\begin{aspt}
\label{aspt:cont_tar}
We require the following assumptions for the source-task-as-representation setting.
\begin{enumerate}[label=(\alph*)]
    \item Given any fixed $y \in \mathcal{Y}_{so}$, $l_{so}(\cdot, y)$ is strongly-convex with constant $c_1$.
    \item Given any fixed $y \in \mathcal{Y}_{ta}$, $\nabla^2 l_{ta}(\cdot, y) \prec c_2$.
    \item Loss function $l_{ta}$ and $l_{so}$ have unbiased gradient, i.e.
    $
        \E[\nabla l(y, y+\epsilon)] = 0 \text{ if } \E[\epsilon] = 0
    $
    \item Any $h_{ta} \in \mathcal{H}_{ta}$ is $c_3$-Lipschitz with respect to $L_2$ distance.
\end{enumerate}
\end{aspt}
\fi

We show that a simple Lipschitz condition on $\mathcal{F}_{ta}$ gives us a bounded transfer-component.

\begin{aspt}[Lipschitz assumption]
\label{aspt:cont_tar}
Any $f_{ta} \in \mathcal{F}_{ta}$ is $L$-Lipschitz with respect to $L_2$ distance.
\end{aspt}

\begin{thm}
\label{thm:source_as_rep}
If Assumption \ref{aspt:cont_tar} holds, task $f_{so}^*$ is $(L, 0)$-transferable to task $f_{ta}^*$ and we have with a high probability,
$$
    \mathcal{E}_{ta}(\hat f_{ta}, \hat h) = \tilde{\mathcal{O}}\left(\frac{L\hat{\mathfrak{G}}_{n_{so}}(\mathcal{H})}{\sqrt{n_{so}}} + \frac{\hat{\mathfrak{G}}_{n_{ta}}(\mathcal{F}_{ta} \circ \hat h)}{\sqrt{n_{ta}}}\right).
$$
\end{thm}
%\begin{proof}
%The proof is given in Appendix %\ref{app:source_as_rep}.
%\end{proof}

Theorem \ref{thm:source_as_rep} bounds the generalization error of two terms. The first term that scales with $1/\sqrt{n_{so}}$ only depends on the complexity of $\mathcal{H}$. Though the second term scales with $1/\sqrt{n_{ta}}$, it is easy to see that $\hat{\mathfrak{G}}_{n_{ta}}(\mathcal{F}_{ta} \circ \hat h) = \hat{\mathfrak{G}}_{n_{ta}}(\mathcal{F}_{ta}) \ll \hat{\mathfrak{G}}_{n_{ta}}(\mathcal{F}_{ta} \circ \mathcal{H})$ with the dataset $\{\hat h(x_{ta, i})\}_{i = 1}^{n_{ta}}$.%, that does not depend on the complexity of representation function space.

==> Representation%20Learning%20(Version%2012650)/sec2_complex_target.tex <==
\subsection{General case}
Previously, we assume that a single source task is a representation of the target task. Now we consider a more general case: there exist  functions in the source prediction space that can be used as representations of the target task. Formally, we consider $\mathcal{F}_{ta} = \mathcal{F}'_{ta} \circ (\mathcal{F}_{so}^{\otimes m})$ for some $m > 0$ and some target-specific function space $\mathcal{F}'_{ta}: \mathcal{Y}_{so}^{\otimes m} \mapsto \mathcal{Y}_{ta}$. Note that $\mathcal{F}_{ta}$ is strictly larger than $\mathcal{F}_{so}$ when $m = 1$ and the identical mapping $x\mapsto x \in \mathcal{F}_{ta}'$. In practice, ResNet \citep{tai2017image} satisfies the above property.

%We first introduce the diversity definition in \cite{tripuraneni2020theory}.

\begin{aspt} 
\label{aspt:2}
Assume any $f'_{ta} \in \mathcal{F}'_{ta}$ is $L'$-Lipschitz with respect to $L_2$ distance.
\end{aspt}

\begin{thm}
\label{thm:general_case}
If Assumption \ref{aspt:2} holds and the source tasks are $(\nu, \mu)$-diverse over its own space $\mathcal{F}_{so}$, then we have 
$$
    \mathcal{E}_{t a}\left(\hat{f}_{t a}, \hat{h}\right)=\tilde{\mathcal{O}}\left(L'm \left(\frac{\nu \hat{\mathfrak{G}}_{Tn_{so}}(\mathcal{F}_{so}^{\otimes T} \circ \mathcal{H})}{\sqrt{Tn_{so}}} + \mu\right) +\frac{\hat{\mathfrak{G}}_{n_{t a}}\left(\mathcal{F}_{ta} \circ \hat{h}\right)}{\sqrt{n_{t a}}}\right).
$$
\end{thm}
%\begin{proof}
%The proof is given in Appendix \ref{app:general_case}.
%\end{proof}

It is shown in \cite{tripuraneni2020theory} that $\hat{\mathfrak{G}}_{{\sum_{s} n_s}}(\mathcal{F}_{so}^{\otimes S} \circ \mathcal{H})$ can be bounded by $\tilde{\mathcal{O}}(\hat{\mathfrak{G}}_{Tn_{so}}(\mathcal{H}) + \sqrt{T}\hat{\mathfrak{G}}_{n_{so}}(\mathcal{F}_{so}))$. Thus, the first term scales with 
$
    {\hat{\mathfrak{G}}_{Tn_{so}}(\mathcal{H})}/{\sqrt{Tn_{so}}} + {\hat{\mathfrak{G}}_{n_{so}}(\mathcal{F}_{so})}/{\sqrt{n_{so}}}.
$
Again the common part shared by all the tasks decreases with $\sqrt{Tn_{so}}$, while the task-specific part scales with $\sqrt{n_{so}}$ or $\sqrt{n_{ta}}$.

\subsection{Applications to deep neural networks}

Theorem \ref{thm:general_case} has a broad range of applications. In the rest of the section, we discuss its application to deep neural networks, where the source tasks are transferred to a target task with a deeper network.%with the same width in terms of the prediction function.

We first introduce the setting for deep neural network prediction function. We consider the regression problem with $\mathcal{Y}_{so} = \mathcal{Y}_{ta} = \mathbb{R}$ and the representation space $\mathcal{Z} \subset \mathbb{R}^{p}$. A depth-$K$ vector-valued neural network is denoted by 
$$
    f(\mathbf{x})=\sigma\left(\mathbf{W}_{K}\left(\sigma\left(\ldots \sigma\left(\mathbf{W}_{1} \mathbf{x}\right)\right)\right)\right),
$$
where each $\mathbf{W}_k$ is a parametric matrix of layer $k$ and $\sigma$ is the activation function. For simplicity, we let $\mathbf{W}_k \in \mathbb{R}^{p \times p}$ for $k = 1, \dots K$. The class of all depth-$K$ neural network is denoted by $\mathcal{M}_K$. We denote the linear class by $\mathcal{L} = \{x \mapsto \alpha^Tx + \beta: \forall \alpha \in \mathbb{R}^p, \|\alpha\|_2 \leq M(\alpha) \}$ for some $M(\alpha) > 0$. We also assume 
$$
    \max\{\|W_k\|_{\infty}, \|W_k\|_{2}\| \} \leq M(k).
$$
where $\|\cdot\|_{\infty}$ and $\|\cdot\|_2$ are the infinity norm and spectral norm. We assume any $z \in \mathcal{Z}, \|z\|_{\infty} \leq D_{Z}$. % Lemma \ref{lem:nn_liptz} shows that any DNN prediction function satisfies Assumption \ref{aspt:2} with constant $L' = M(\alpha)\Pi_{k = 1}^KM(k)$.


\paragraph{Deeper network for the target task.} We now consider the source task with prediction function of a depth-$K_{so}$ neural network followed by a linear mapping and target task with depth-$K_{ta}$ neural network. We let $K_{ta} > K_{so}$. Then we have 
$$
    \mathcal{F}_{ta} = \mathcal{L} \circ \mathcal{M}_{K_{ta} - K_{so}} \circ \mathcal{M}_{K_{so}} \text{ and } \mathcal{F}_{so} = \mathcal{L} \circ \mathcal{M}_{K_{so}}.
$$

\iffalse
\begin{figure}[ht]
    \centering
    \floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=4cm}}]{figure}[\FBwidth]
{\caption{An illustration of how to view the target network with $p$ source tasks as a representation. We choose the coefficient of the $p$ linear mappings, such that $(\alpha_1, \dots, \alpha_p) = W^*_{K_{so} + 1}$, the true parameters in the $K_{so}+1$-th layer of the target task.}\label{fig:test}}
    {\includegraphics[width = 0.6\textwidth]{Figures/Figure2.png}}
    \label{fig:network_illus}
\end{figure}
\fi

%As shown in Figure \ref{fig:network_illus}, for any target prediction function $f_{ta}^*$, we can find $p$ prediction functions $f_{1}', \dots, f_{p}'$ in $\mathcal{F}_{so}$ such that $f_{ta}^*(z) = f'\circ m' \circ \sigma (f_1'(z), \dots, f_p'(z))$ for some $f' \in \mathcal{L}, m'\in \mathcal{M}_{K_{ta} - K_{so} - 1}$. 
Using the fact that $\mathcal{M}_1 = \sigma(\mathcal{L}^{\otimes p})$, we can write $\mathcal{F}_{ta}$ as $\mathcal{L}\circ \mathcal{M}_{K_{ta} - K_{so} - 1} \circ \sigma \circ (\mathcal{F}_{so}^{\otimes p})$. Thus, we can apply Theorem \ref{thm:general_case} and the standard Gaussian complexity bound for DNN models, which gives us Corollary \ref{cor:deep_application}.

\begin{cor}
\label{cor:deep_application}
Let $\mathcal{F}_{so}$ be depth-$K_{so}$ neural network and $\mathcal{F}_{ta}$ be depth-$K_{ta}$ neural network. If source tasks are $(\nu, 0)$-diverse over $\mathcal{F}_{so}$, we have 
\begin{align*}
    &\mathcal{E}_{t a}\left(\hat{f}_{t a}, \hat{h}\right)= \\
 &\tilde{\mathcal{O}}\left({p\nu M(\alpha) \Pi_{k=1}^{K_{ta}}M(k)}\left( \frac{\hat{\mathfrak{G}}_{Tn_{so}}(\mathcal{H})}{\sqrt{Tn_{so}}} + \frac{D_{Z}\sqrt{K_{so}}}{\sqrt{n_{so}}}\right)+\frac{ D_{Z} \sqrt{K_{ta}} \cdot M(\alpha) \Pi_{k = 1}^{K_{ta}}M(k)}{\sqrt{n_{ta}}}\right). \numberthis \label{equ:dnn_bound}
\end{align*}

%\begin{proof}
%The proof of Corollary \ref{cor:deep_application} is given by Appendix \ref{app:deep_application}.
%\end{proof}
%Note that if $n_{so} = n_{ta} = n$, the bound becomes
%$$
%    \tilde{\mathcal{O}}\left({p \nu \Pi_{k=K_{so}+2}^{K_{ta}}M(k)}\left(\frac{\hat{\mathfrak{G}}_{T n}(\mathcal{H})}{Tn}\right)+(\frac{p \nu}{M(K_{so} + 1)} + 1)\left(\frac{ D_{Z} \sqrt{K_{ta}} \cdot M(\alpha) \Pi_{k = 1}^{K_{ta}}M(k)}{\sqrt{n}}\right)\right).
%$$
\end{cor}

Note that the terms that scales with $1/\sqrt{n_{so}}$ and $1/\sqrt{n_{ta}}$ have similar coefficients $M(\alpha) \Pi_{k = 1}^{K_{ta}}M(k)$, which do not depends on the complexity of $\mathcal{H}$. The term that depends on $\hat{\mathfrak{G}}_{T n_{so}}(\mathcal{H})$ scales with $1/\sqrt{Tn_{so}}$ as we expected. %has an extra coefficient on $p \nu \Pi_{k=K_{so}+2}^{K_{ta}}M(k)$, which is a result of transferring from depth $K_{so}$ to depth $K_{ta}$ networks.



%\paragraph{Source tasks have more layers.} \ziping{Make this a simple discussion.}
%A trivial result is that when $\mathcal{H}_{so} = \mathcal{H}_{so}' \circ (\mathcal{H}_{ta}^{\otimes m})$ for some positive integer $m$, then if $x \mapsto x \in \mathcal{H}_{so}'$, we have $\mathcal{H}_{ta} \subset \mathcal{H}_{so}$. Then diversity over $\mathcal{H}_{so}$ directly implies diversity over $\mathcal{H}_{ta}$.

%In the DNN applications, ResNet (add citation) satisfies the property.

\iffalse
\subsection{Diversity of DNN prediction functions} 
Now we discuss the diversity of DNN prediction functions. To have $\epsilon = 0$, we will need $d^{K_{so}}$ source tasks. However, we can discuss the convex hull approximation and have a dimension independent bound.

\ziping{Points I wanna make but haven't find a place for it: 1) in a lot of applications the diversity does not depend on the representation part. It is solely determined by the prediction functions.}

\begin{thm}
There exists $d^K$ functions in depth-$K$ NN class such that they are $(\nu, \mu)$-diverse over the depth-$K$ NN class with square loss.
\end{thm}
\begin{proof}
ss
\end{proof}

\paragraph{A general condition for diversity.} Assume that target class can be approximated by a basis $\phi_1(\cdot), \dots, \phi_d(\cdot)$ with an approximation error $\epsilon$, then $d$ sources can be diverse over the target function class with constants $(1/d, \epsilon)$.

Consider Fourier series, Taylor series and other approximation approach.

Actually, this might be the special case of the RKHS 

\url{https://en.wikipedia.org/wiki/Reproducing_kernel_Hilbert_space}

\url{https://stats385.github.io/assets/lectures/lecture6_stats385_stanford_nov17.pdf}

\paragraph{Wider network for the target task.}
Instead of using a deeper network, another choice of increasing the network complexity is to use a wider network. We consider a special case, where the prediction function for both source and target tasks are depth-1 neural network followed by a linear mapping. The number of hidden units is $p_{so}$ and $p_{ta}$ for source and target tasks, respectively.

To proceed, we use the following trick: there exists a function in $\mathcal{H}_{so}$, which is a representation of the prediction function $h^*_{ta}$ of the target task. We illustrate the trick in Figure \ref{fig:trick_illustrated}.

\begin{figure}[H]
    \centering
\includegraphics[width = 0.9\textwidth]{Figures/Figure1.png}
    \caption{The figure illustrates that a wider network of $p_{ta}$ units could be seen as a network of $p_{ta} - p_{so}$ units built on a representation of the network with $p_{so}$ units.}
    \label{fig:trick_illustrated}
\end{figure}

\begin{thm}
If source tasks are $(\nu, 0)$-diverse over $\mathcal{H}_{so}$, we have 
$$
    G_{t a}\left(\hat{h}_{t a}, \hat{g}\right)=\tilde{\mathcal{O}}\left({\nu M \|W(p_{ta}-p_{so})\|_{2, \infty}}\left(\frac{\hat{\mathfrak{G}}_{\sum_{s} n_{s}}(\mathcal{G})}{\sum_{s} n_{s}}+\frac{p \cdot D \sqrt{K_{so}} \cdot  M^{K_{so}}}{\sqrt{\bar n_{so}}}\right)+\frac{p \cdot D \sqrt{K_{ta}} \cdot M^{K_{ta}}}{\sqrt{n_{ta}}}\right),
$$
where $W(p_{ta}-p_{so})$ is the parameters for the last $p_{ta} - p_{so}$ units.
\end{thm}
\paragraph{Linear or Logistic or DNN prediction functions}
We first show that our framework replicates the results under linear prediction functions with a weaker assumption compared to previous works \cite{du2020few}.

Sufficient conditions for 
\begin{enumerate}
    \item arbitrary task-specific function (convexity? Linear function we can directly prove but what is the case in the general class?) It could naturally generalize to any target class that is larger than the source class because we can find one function in source class that is a representation of the target one. In this case, we don't need convexity!!!
    \item arbitrary feature distribution
    \item general task source prediction functions?
\end{enumerate}
\fi

==> Representation%20Learning%20(Version%2012650)/sec3_diversity_general_case.tex <==
\section{Diversity of non-linear function classes}
\label{sec:div_general}

%\ziping{Generalize to different activation functions.}
While Corollary \ref{cor:deep_application} considers the nonlinear DNN prediction function space under a diversity condition, it is not clearly understood how diversity can be achieved for nonlinear spaces. In this section, we first discuss a specific non-linear prediction function space and show a fundamental barrier to achieving diversity. Then we extend our result to general function classes by connecting eluder dimension and diversity. We end the section with positive results for achieving diversity under a generalized rank condition. %\ambuj{I rewrote this para so please check! Ziping: Looks good!}

We consider a subset of depth-1 neural networks with ReLu activation function: $\mathcal{F} = \{x \mapsto [\langle x, w \rangle - (1-\epsilon/2)]_{+}: \|x\|_2 \leq 1, \|w\|\leq 1\}$ for some $\epsilon > 0$. Our lower bound construction is inspired by the similar construction in Theorem 5.1 of \cite{dong2021provable}.
\begin{thm}
\label{thm:ReLu_hard_case}
Let $\mathcal{T} = \{f_1, \dots, f_T\}$ be any set of depth-1 neural networks with ReLu activation in $\mathcal{F}$. For any $\epsilon > 0$, if $T \leq 2^{d \log(1/\epsilon) - 1}$, there exists some representation $h^*, h' \in \mathcal{H}$, some distribution $P_{X}$ and a target function $f_{ta}^* \in \mathcal{F}$, such that
$$
    \inf_{\vect{f} \in \mathcal{F}}\mathcal{E}_{so}(\vect{f}, h') = 0,\quad \text{while } \inf_{{f} \in \mathcal{F}}\mathcal{E}_{ta}(f, h') = \epsilon^2/32.
$$
\end{thm}
%\begin{proof}
%The proof is given by Appendix \ref{app:more_activation_funcs}.
%\end{proof}

Theorem \ref{thm:ReLu_hard_case} implies that we need at least $\Omega({2^{d}\log(1/\epsilon)})$ source tasks to achieve diversity. Otherwise, we can always find a set of source tasks and a target task such that the generalization error in source tasks are minimized to 0 while that in target task is $\epsilon^2 / 32$. Though ReLu gives us a more intuitive result, we do show that similar lower bounds can be shown for other popular activation functions, for example, sigmoid function (see Appendix \ref{app:more_activation_funcs}).

\subsection{Lower bound using eluder dimension}
We extend our result by considering a general function space $\mathcal{F}$ and build an interesting connection between diversity and eluder dimension \citep{russo2013eluder}. We believe we are the first to notice a connection between eluder dimension and transfer learning.

Eluder dimension has been used to measure the sample complexity in the Reinforcement Learning problem. It considers the minimum number of \textit{inputs}, such that any two functions evaluated similarly at these inputs will also be similar at any other input. However, diversity considers the minimum number of functions such that any two representations with similar \textit{outputs} for these functions will also have similar output for any other functions. Thus, there is a kind of duality between eluder dimension and diversity.

We first formally define eluder dimension. Let $\mathcal{F}$ be a function space with support $\mathcal{X}$ and let $\epsilon > 0$.
\begin{defn}[($\mathcal{F}, \epsilon$)-dependence and eluder dimension (\cite{osband2014model})]
We say that $x \in \mathcal{X}$ is $(\mathcal{F}, \epsilon)$-dependent on $\{x_1, \dots, x_n\} \subset \mathcal{X}$ iff $$
    \forall f, \tilde{f} \in \mathcal{F}, \quad \sum_{i=1}^{n}\left\|f\left(x_{i}\right)-\tilde{f}\left(x_{i}\right)\right\|_{2}^{2} \leq \epsilon^{2} \Longrightarrow\|f(x)-\tilde{f}(x)\|_{2} \leq \epsilon.
$$
We say $x \in \mathcal{X}$ is $(\mathcal{F}, \epsilon)$-independent of $\{x_1, \dots, x_n\}$ iff it does not satisfy the definition of dependence.

The eluder dimension $\operatorname{dim}_E(\mathcal{F}, \epsilon)$ is the length of the longest possible sequence of elements in $\mathcal{X}$ such that for some $\epsilon' \geq \epsilon$ every element is $(\mathcal{F}, \epsilon')$-independent of its predecessors.

We slightly change the definition and let $\operatorname{dim}^{s}_E(\mathcal{F}, \epsilon)$ be the shortest sequence such that any $x \in \mathcal{X}$ is $(\mathcal{F}, \epsilon)$-dependent on the sequence. 
\end{defn}

% Note that we introduce this definition so as to avoid extreme cases, for example, $\mathcal{F} = \mathcal{F}_1 \cup \mathcal{F}_2$ and $\mathcal{F}_1$ is more complex than $\mathcal{F}_2$. The original definition cares about the worst case, i.e. the complexity of $\mathcal{F}_1$, while we care about the lowest number of functions that can cover the whole space, so our measure will be closer to the complexity of $\mathcal{F}_2$. 
Although $dim_{E}^s(\mathcal{F}, \epsilon) \leq dim_{E}(\mathcal{F}, \epsilon)$, it can be shown that in many regular cases, say linear case and generalized linear case, $dim_{E}(\mathcal{F}, \epsilon)$ is only larger then $dim_{E}^s(\mathcal{F}, \epsilon)$ up to a constant. %Indeed, we propose $dim^{+}_E$ to avoid some extreme case, where $\mathcal{F} = \mathcal{F}_1 \cup \mathcal{F}_2$.

% A simple way to construct diverse source tasks is to start with an empty set and keep adding tasks which current set could not transfer to until we can not find any such task. Let $i$ be the current step, any task with $\nu = \mathcal{O}(i)$ should be considered transferable because any task that is already in the set has $\nu = i$ in the worst case. The following Theorem states that such process should be longer than the eluder dimension of $\mathcal{F}^*$.

\begin{thm}
\label{thm:eluder}
For any function class $\mathcal{F}:\mathcal{X} \mapsto \mathbb{R}$, and some $\epsilon > 0$, let $\mathcal{F}^*$ be the dual class of $\mathcal{F}$. Let $d_E = \operatorname{dim}^s_E(\mathcal{F}^*, \epsilon)$. Then for any sequence of tasks $f_1, \dots, f_{t}$, $t \leq d_E-1$, there exists a task $f_{t+1} \in \mathcal{F}$ such that for some data distribution $P_X$ and two representations $h$, $h^*$, %\ziping{use $h, h^*$}
%$$
%    \frac{1}{t}\inf_{f'_1, \dots, f'_{t} }\sum_{i = 1}^{t}\E_X \|f'_i(g(X)) - f_i(g^*(X))\|_2^2 \leq \frac{\epsilon^2}{2t}, \text{ while } \inf_{f'_{t+1} \in \mathcal{F}}\E_X \|f'_{t+1}(g(X)) - f_{t+1}(g^*(X))\|_2^2 > \frac{\epsilon^2}{4},
%$$
%which gives
$$
\frac{\inf_{f'_{t+1} \in \mathcal{F}}\E_X \|f'_{t+1}(h(X)) - f_{t+1}(h^*(X))\|_2^2}{\frac{1}{t}\inf_{f'_1, \dots, f'_{t} }\sum_{i = 1}^{t}\E_X \|f'_i(h(X)) - f_i(h^*(X))\|_2^2} \geq t/2.
$$
\end{thm}
%\begin{proof}
%The proof is given by Appendix \ref{app:eluder}.
%\end{proof}

Theorem \ref{thm:eluder} formally describes the connections between eluder dimension and diversity. To interpret the theorem, we first discuss what are good source tasks. Any $T$ source tasks that are diverse could transfer well to a target task if the parameter $\nu$ could be bounded by some fixed value that is not increasing with $T$. For instance, in the linear case, $\nu = \mathcal{O}(d)$ no matter how large $T$ is. While for a finite function class, in the worst case, $\nu$ will increase with $T$ before $T$ reaches $|\mathcal{F}|$. Theorem \ref{thm:eluder} states that if the eluder dimension of the dual space is at least $d_E$, then $\nu$ scales with $T$ until $T$ reaches $d_E$, as if the function space $\mathcal{F}$ is discrete with $d_E$ elements.

Note that this result is consistent with what is shown in Theorem \ref{thm:general_hard_case} as eluder dimension of the class discussed above is lower bounded by $\Omega(2^{d})$ as well \cite{li2021eluder}.

\subsection{Upper bound using approximate generalized rank}
Though we showed that diversity is hard to achieve in some nonlinear function class, we point out that diversity can be easy to achieve if we restrict the target prediction function such that they can be realized by linear combinations of some known basis. \cite{tripuraneni2020theory} has shown that any source tasks $f_1, \dots, f_T \in \mathcal{F}$ are $(1/T, \mu)$-diverse over the space $\{f \in \mathcal{F}: \exists \tilde{f} \in \operatorname{conv}(f_1, \dots, f_T) \text{ such that } \sup_{z}\|f(z) - \tilde{f}(z)\|\leq \mu\}$, where $\operatorname{conv}(f_1, \dots, f_T)$ is the convex hull of $\{f_1, \dots, f_T\}$. This can be characterized by a complexity measure, called generalized rank. Generalized rank is the smallest dimension required to embed the input space such that all hypotheses in a function class can be realizable as halfspaces. Generalized rank has close connections to eluder dimension. As shown in \cite{li2021eluder}, eluder dimension can be upper bounded by generalized rank. %\ziping{Make it clear why this is not conflicting with the previous results.}

\begin{defn}[Approximate generalized rank with identity activation] Let  $\mathcal{B}_d(R) \coloneqq \{x\in\mathbb{R}^d \mid \|x\|_2 \leq R\}$. The $\mu$-approximate $\operatorname{id-rk}(\mathcal{F, R})$ of a function class $\mathcal{F}:\mathcal{X} \mapsto \mathbb{R}$ at scale $R$ is the smallest dimension $d$ for which there exists mappings $\phi:\mathcal{X} \mapsto \mathcal{B}_d(1)$ and $w:\mathcal{F}\mapsto\mathcal{B}_d(R)$ such that $$
    \text{for all } (x, f) \in \mathcal{X} \times \mathcal{F}: |f(x) - \langle w(f), \phi(x) \rangle| \leq \mu.
$$
\end{defn}

\begin{prop}
\label{prop:gr}
For any $\mathcal{F}$ with $\mu$-approximate $\operatorname{id-rank}(\mathcal{F}, R) \leq d_i$ for some $R > 0$, there exists no more than $d_i$ functions, $f_1, \dots, f_{d_i}$, such that $w(f_1), \dots w(f_{d_i})$ span $\mathbb{R}^{d_{d_i}}$. Then $f_1, \dots, f_{d_i}$ are $(d_i, \mu)$-diverse over $\mathcal{F}$.
\end{prop}

Proposition \ref{prop:gr} is a direct application of Lemma 7 in \cite{tripuraneni2020theory}. Upper bounding $\text{id-rank}$ is hard for general function class. However, this notation can be useful for those function spaces with a known set of basis functions. For example, any function space $\mathcal{F}$ that is square-integrable has a Fourier basis. Though the basis is an infinite set, we can choose a truncation level $d$ such that the truncation errors of all functions are less than $\mu$. Then the hypothesis space $\mathcal{F}$ has $\mu$-approximate $\operatorname{id-rank}$ less than $d$.
% In general, this supports the common practice of keeping all the layers except for the last linear mapping, to ensure $\mathcal{F}_{so}$ is simple linear mapping. Some \ziping{Add reference} papers suggest that keeping different number of layers extracts different levels of representation. In these cases, the target prediction function $f_{ta}^*$ should not be an arbitrary function in the class. Instead, $\mathcal{F}_{ta}$ may be restricted around $f_{t}^*$'s such that the diversity over $\mathcal{F}_{ta}$ holds. An example would be $\mathcal{F}_{ta} = \{\text{any } f: \exists \alpha_1, \dots, \alpha_T, \|f - \sum_{t = 1}^T \alpha_t f_t^*\|_2 \leq \epsilon \}$. This example has been discussed in \cite{tripuraneni2020theory}.

% \ziping{The results still hold even if the target function class is simpler!}
%Then we give a general condition for sufficiency of diversity and we show that ResNet satisfies the condition.

% In general, the main conclusion of this section is that we shall use simple tasks to learn representation so as to generalize to hard tasks.

\iffalse
\paragraph{Results from bounded functions.} Note that any square-integrable function space has a Schauder basis. Define 
$$\mathcal{C}_k = 
    \{\sqrt{2} \sin (2 \pi n x) \mid n = 1, \dots k\} \cup\{\sqrt{2} \cos (2 \pi n x) \mid n = 1, \dots k\} \cup\{1\}.
$$
Without loss of generality, for $L^2[0, 1]$, the collection $\mathcal{C}_\infty$ forms a basis, i.e. any $f \in L^2[0, 1]$ can be written as $f(x) = \sum_{c \in \mathcal{C}_{\infty}}^\infty \alpha_c c(x)$. 
\begin{thm}
Now let each source tasks use a basis from $C_k$. If the target prediction function $f$ satisfies $\sum_{c \not\in C_k} |\alpha_c| \leq \epsilon$, then the source tasks are $(1/|C_k|, \epsilon)$-diverse over the class of the target prediction function.
\end{thm}
\begin{proof}
We mainly use the fact in \cite{tripuraneni2020theory}.
\end{proof}
\fi

==> Representation%20Learning%20(Version%2012650)/sec4_multiclass_as_multitask.tex <==



==> Representation%20Learning%20(Version%2012650)/sec5_simulation.tex <==

\section{Experiments}
%\ambuj{I know you're short on space and want to keep this short. But it is currently also not very clear. We need to be concise: that is, short *and* clear.}

In this section, we use simulated environments to evaluate the actual performance of representation learning on DNNs trained with gradient-based optimization methods. We also test the impact of various hyperparameters. Our results indicate that even though our theory is shown to hold for ERM estimators, their qualitative theoretical predictions still hold when Adam is applied and the global minima might not be found. Before we introduce our experimental setups, we discuss a difference between our theories and experiments: our experiments use a single regression task with multiple outputs as the source task, while our analyses are built on multiple source tasks. 

\subsection{Diversity of problems with multiple outputs}
%\label{sec:multiclass}

Though we have been discussing achieving diversity from multiple source tasks, we may only have access to a single source task in many real applications, for example, ImageNet, which is also the case in our simulations. In fact, we can show that diversity can be achieved by a single multiclass classification or multivariate regression source task. The diversity for the single multi-variate regression problem with L2 loss is trivial as the loss function is decomposable. For multi-class classification problems or regression problems with other loss functions, we will need some assumptions on boundedness and continuous. We refer the readers to Appendix \ref{app:multi_output} for details. 


\subsection{Experiments setup} 

Our four experiments are designed for the following goals. The first two experiments (Figure \ref{fig:simulations}, a and b) target on the actual dependence on $n_{so}, n_{ta}, K_{so}$ and $K_{ta}$ in Equation (\ref{equ:dnn_bound}) that upper bounds the errors of DNN prediction functions. Though the importance of diversity has been emphasized by various theories, no one has empirically shown its benefits over random tasks selection, which we explore in our third experiment (Figure \ref{fig:simulations}, c). Our fourth experiment (Figure \ref{fig:simulations}, d) verifies the theoretical negative results of nonlinearity of source prediction functions showed in Theorem \ref{thm:ReLu_hard_case} and \ref{thm:eluder}. 

Though the hyper-parameters vary in different experiments, our main setting can be summarized below. We consider DNN models of different layers for both source and target tasks. The first $K$ layers are the shared representation. The source task is a multi-variate regression problem with output dimension $p$ and $K_{so}$ layers following the representation. The target task is a single-output regression problem with $K_{ta}$ layers following the representation. We used the same number of units for all the layers, which we denote by $n_u$. 
A representation is first trained on the source task using $n_{so}$ random samples and is fixed for the target task, trained on $n_{ta}$ random samples. In contrast, the baseline method trains the target task directly on the same $n_{ta}$ samples without the pretrained network. We use Adam with default parameters for all the training. We use MSE (Mean Square Error) to evaluate the performance under different settings.

\iffalse
\begin{figure}[ht]
    \centering
\includegraphics[width = 0.9\textwidth]{Figures/simulations/network.png}
    \caption{An example of DNNs used in the experiments. We use $K = 5$ layers for the shared representation, $K_{so} = K_{ta} = 1$ layer for the prediction functions. The number of units are set to be 4 for all the layers. The number of outputs is 4 and 1 in source and target task, respectively.}
    \label{fig:illustration}
\end{figure}
\fi


\subsection{Results} 

Figure \ref{fig:simulations} summaries our four experiments, with all the Y axes representing the average MSE's of 100 independent runs with an error bar showing the standard deviation. The X axis varies depending on the goal of each experiment. In subfigure (a), we test the effects of the numbers of observations for both source and target tasks, while setting other hyperparameters by default values. The X axis represents $n_{so}$ and the colors represents $n_{ta}$. In subfigure (b), we test the effects of the number of shared representation layers $K$. To have comparable MSE's, we keep the sum $K + K_{ta} = 6$ and run $K = 1, \dots, 5$ reflected in the X axis, while keeping $K_{so} = 1$. In subfigure (c), we test the effects of diversity. The larger $p$ we have, the more diverse the source task is. We keep the actual number of observations $n_{so} \cdot p = 4000$ for a fair comparison. Lastly, in subfigure (d), we test whether diversity is hard to achieve when the source prediction function is nonlinear. The X axis is the number of layers in source prediction function $K_{so}$. The nonlinearity increases with $K_{so}$. We run $K_{so} = 1, 2, 3$ and add an activation function right before the output such that the function is nonlinear even if $K_{so} = 1$. %\ambuj{rewrite last sentence}


\begin{figure}[htb]
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width = 1\textwidth]{Figures/simulations/Simulation_n_effects.pdf}
    \caption{Effects of sample sizes}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width = 1\textwidth]{Figures/simulations/Simulation_layer_effects.pdf}
    \caption{Effects of $K$}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width = 1\textwidth]{Figures/simulations/Simulation_diverse_effects.pdf}
    \caption{Effects of diversity}
    \end{subfigure}
    \begin{subfigure}[b]{0.45\textwidth}
    \includegraphics[width = 1\textwidth]{Figures/simulations/Simulation_hardness_effects.pdf}
    \caption{Effects of $K_{so}$}
    \end{subfigure}
    \caption{\textbf{(a)} Effects of the numbers of observations for both source ($n_{so}$) and target tasks ($n_{ta}$). \textbf{(b)} Effects of the number of shared representation layers $K$. %We keep the total $K + K_{ta} = 6$ and run $K = 1,\dots, 5$ (X axis), while keeping $K_{so} = 1$. 
    \textbf{(c)} Effects of diversity determined by the output dimensions $p$. We keep the actual number of observations $n_{so} \cdot p = 4000$. \textbf{(d)} Effects of nonlinearity of the source prediction function. Higher $K_{so}$ indicates higher nonlinearity.}
    \label{fig:simulations}
\end{figure}

\iffalse
Our four experiments plays with the following hyperparameters: 1) number of observations, i.e. $n_{so}$ and $n_{ta}$; 2) number of layers $K_{ta}$ in target prediction function; 3) effects of diversity initialization; 4) performance when $K_{so} \geq 1$.  Now we describe the setup for each experiment in more details.
\begin{enumerate}
    \item \textbf{Experiment 1:} we try the different combinations of $n_{so} = \{100, 1000, 10000\}$ and $n_{ta} = \{10, 100, 1000\}$, while fixing $K = 5$ and $K_{so} = K_{ta} = 0$ (linear mapping without any activation).
    \item \textbf{Experiment 2:} we fix a depth-7 DNN for the target task, i.e. $K + K_{ta} = 7$. We change the depth of the source task from $1$ to $15$ with an increment $2$. The number of shared layers $K = 1, 3, 5, 7, 7, 7, 7$. In other words, when the source task have less layers, we use all the layers in the source task as representation. Otherwise, we use 7 layers as representation. Note that $K_{so}$ is always 0.
    \item \textbf{Experiment 3: } we let the number of output $p$ for the source tasks change from 1 to 4 for an 4-unit depth-5 neural network. The number of observations is $4000 / p$ such that the total numbers of outputs are the same. The true parameters of the source prediction functions are initialized diversely, i.e. the linear mapping matrices have orthogonal columns.
    \item \textbf{Experiment 4: } we test the decrease in the benefits of representation learning when $K_{so}$ increases. 
\end{enumerate}
\fi

In Figure \ref{fig:simulations} (a), MSE's decrease with larger numbers of observations in both source and target tasks, while there is no significant difference between $n_{so} = 1000$ and $10000$. The baseline method without representation learning performs worst and it performs almost the same when $n_{ta}$ reaches 1000. In (b), there are positive benefits for all different numbers of the shared layers and the MSE is the lowest at 5 shared layers. As shown in Figure \ref{fig:simulations} (c), the MSE's and their variances are decreasing when the numbers of outputs increase, i.e., higher diversity. Figure \ref{fig:simulations} (d) shows that there is no significant difference between baseline and $K_{so} = 1, 2, 3$. When $K_{so} = 2, 3$ there is a negative effects. %However, when the number of layers reaches 2 and 3, we have negative transfer.
 
\section{Discussions}
\label{sec:discussion}
In this paper, we studied representation learning beyond linear prediction functions. We showed that the learned representation can generalize to tasks with multi-layer neural networks as prediction functions as long as the source tasks use linear prediction functions. We show the hardness of being diverse when the source tasks are using nonlinear prediction functions by giving a lower bound on the number of source tasks in terms of eluder dimension. We further give an upper bound depending on the generalized rank. 

Focusing on future work, we need better tools to understand the  recently proposed complexity measure generalized rank. Our analyses rely on the ERM, while in practice as well as in our simulations, gradient-based optimization algorithms are used. Further analyses on the benefits of representation learning that align with practice on the choice of optimization method should be studied. Our analyses assume arbitrary source tasks selection, while, in real applications, we may have limited data from groups that are under represented, which may lead to potential unfairness. Algorithm that calibrates this potential unfairness should be studied.
 %\ziping{Add conclusion on the other method, say boosting}

% \ambuj{conclusion needs to be better. future work needs to be added.}

\newpage

==> Representation%20Learning%20(Version%2012650)/sec_introduction.tex <==

\begin{abstract}
Recent papers on the theory of representation learning has shown the importance of a quantity called diversity when generalizing from a set of source tasks to a target task. Most of these papers assume that the function mapping shared representations to predictions is linear, for both source and target tasks. In practice, researchers in deep learning use different numbers of extra layers following the pretrained model based on the difficulty of the new task. This motivates us to ask whether diversity can be achieved when source tasks and the target task use different prediction function spaces beyond linear functions. We show that diversity holds even if the target task uses a neural network with multiple layers, as long as source tasks use linear functions. If source tasks use nonlinear prediction functions, we provide a negative result by showing that depth-1 neural networks with ReLu activation function need exponentially many source tasks to achieve diversity. For a general function class, we find that eluder dimension gives a lower bound on the number of tasks required for diversity. Our theoretical results imply that simpler tasks generalize better. Though our theoretical results are shown for the global minimizer of empirical risks, their qualitative predictions still hold true for gradient-based optimization algorithms as verified by our simulations on deep neural networks.
\end{abstract}

\section{Introduction}
It has become a common practice \citep{tan2018survey} to use a pre-trained network as the representation for a new task with $\textit{small}$ sample size in various areas including computer vision \citep{marmanis2015deep}, speech recognition \citep{dahl2011context,jaitly2012application,howard2018universal} and machine translation \citep{weng2020acquiring}. Most representation learning is based on the assumption that the source tasks and the target task share the same low-dimensional representation.

In this paper, we follow the previous work \citep{tripuraneni2020theory} on representation learning by assuming each task, labeled by $t$, generates observations noisily from the mean function $f_t^* \circ h^*$, where $h^*$ is the true representation shared by all the tasks and $f_t^*$ is called the prediction function. We assume $h^* \in \mathcal{H}$, the representation function space and $f_t \in \mathcal{F}_t$, the prediction function space.
%We assume $h^* \in \mathcal{H}$ and $f_t \in \mathcal{F}_t$ for the representation function space $\mathcal{H}$ and the prediction function space $\mathcal{F}_t$.
\cite{tripuraneni2020theory} proposed a diversity condition which guarantees that the learned representation will generalize to target tasks with any prediction function. Assume we have $T$ source tasks labeled by $1, \dots, T$ and $\mathcal{F}_1 = \dots = \mathcal{F}_T = \mathcal{F}_{so}$. We denote the target task by $ta$ and let $\mathcal{E}_t(f, h)\in \mathbb{R}$ be the excess error of $f, h \in \mathcal{F}_t \times \mathcal{H}$ for task $t$. The diversity condition can be stated as follows: there exists some $\nu > 0$, such that for any $f_{ta}^* \in \mathcal{F}_{ta}$ and any $h \in \mathcal{H}$,
$$
    %\sup_{f^*_{ta} \in \mathcal{F}_{ta}}
    \underset{\text{Excess error given $h$ for target task}}{\inf_{ f_{ta} \in \mathcal{F}_{ta}}\mathcal{E}_{ta}( f_{ta}, h)}  \leq \nu \underset{\text{Excess error given $h$ for source tasks}}{\inf_{ f_t \in \mathcal{F}_{so}, t = 1, \dots, T} \frac{1}{T}\sum_{t = 1}^T\mathcal{E}_t( f_t, h)}.  %\text{ for all } h \in \mathcal{H}. 
$$
The diversity condition relates the excess error for source tasks and the target task with respect to any fixed representation $h$. A smaller $\nu$ indicates a better transfer from source tasks to the target task. Generally, we say $T$ source tasks achieve diversity over $\mathcal{F}_{ta}$ when $\nu$ is finite and relatively small. 

The number of source tasks plays an important role here. To see this, assume $\mathcal{F}_{so} = \mathcal{F}_{ta} = \mathcal{F}$ is a discrete function space and each function can be arbitrarily different. In this case, we will need the target task to be the same as at least one source task, which in turn requires $T \geq |\mathcal{F}|$ and $\nu \geq |\mathcal{F}|$. So far, it has only been understood that when \textit{both} source tasks and target task use \textit{linear} prediction functions, it takes at least $d$ source tasks to be diverse, where $d$ is the number of dimension of the linear mappings. This paper answers the following two open questions with a focus on the deep neural network (DNN) models:
$$
\begin{array}{cc}
     \textit{How does representation learning work when $\mathcal{F}_{so} \neq \mathcal{F}_{ta}$?}\\
     \textit{How many source tasks do we need to achieve diversity with nonlinear prediction functions?}  
\end{array}
$$
%Our focus will be on the above two questions under deep neural network prediction functions.

There are strong practical motivations to answer the above two questions. In practice, researchers use representation learning despite the difference in difficulty levels of source and target tasks. We use a more complex function class for substantially harder target task, which means $\mathcal{F}_{so} \neq \mathcal{F}_{ta}$. This can be reflected as extra layers when a deep neural network model is used as prediction functions.  On the other hand, the source task and target task may have different objectives. Representation pretrained on a classification problem, say ImageNet, may be applied to object detection or instance segmentation problems. For instance, \citet{oquab2014learning} trained a DNN on ImageNet and kept all the layers as the representation except for the last linear mapping, while two fully connected layers are used for the target task on object detection.

Another motivation for our work is the mismatch between recently developed theories in representation learning and the common practice in empirical studies. Recent papers on the theory of representation learning all require multiple sources tasks to achieve diversity so as to generalize to any target task in $\mathcal{F}$ \citep{maurer2016benefit,du2020few,tripuraneni2020theory}. However, most pretrained networks are only trained on a single task, for example, the ImageNet pretrained network. To this end, we will show that a single multi-class classification problem can be diverse.

Lastly, while it is common to simply use linear mapping as the source prediction function, there is no clear theoretical analysis showing whether or not diversity can be achieved with \textit{nonlinear} prediction function spaces.  %In this paper, we connects the eluder dimension \cite{russo2013eluder,osband2014model} to the diversity by showing that large eluder dimension of dual space of $\mathcal{F}_{so}$ implies large number of source tasks required.
%\ziping{Add a little about the challenge of the problems.}

\paragraph{Main contributions.}
We summarize the main contributions made by this paper.
\begin{enumerate}
    \item We show that diversity over $\mathcal{F}_{so}$ implies diversity over  $\mathcal{F}_{ta}$, when both $\mathcal{F}_{so}$ and $\mathcal{F}_{ta}$ are DNNs and $\mathcal{F}_{ta}$ has more layers. More generally, the same statement holds when $\mathcal{F}_{ta}$ is more complicated than $\mathcal{F}_{so}$, in the way that $\mathcal{F}_{ta} = \mathcal{F}'_{ta} \circ (\mathcal{F}_{so}^{\otimes m})$ for some positive integer $m$\footnote{$\mathcal{F}^{\otimes T}$ is the $T$ times Cartesian product of $\mathcal{F}$.} and function class $\mathcal{F}_{ta}'$.
    \item Turning our attention to the  analysis of diversity for non-linear prediction function spaces, we show that for a depth-1 NN, it requires $\Omega(2^{d})$ many source tasks to establish diversity with $d$ being the representation dimension. For general  $\mathcal{F}_{so}$, we provide a lower bound on the number of source tasks required to achieve diversity using the eluder dimension \citep{russo2013eluder} and provide a upper bound using the generalized rank \citep{li2021eluder}.
    %\item We show that a single multiclass classification problem with $T$ classes can be diverse.
    \item We show that, from the perspective of achieving diversity, a single source task with multiple outputs can be equivalent to multiple source tasks. While our theories are built on empirical risk minimization, our simulations on DNNs for a multi-variate regression problem show that the general statement still hold when a stochastic gradient descent is used for optimization. %\ziping{Also mention the multiple output point.}
\end{enumerate}
% Our various theoretical contributions justify a common practice using pretrained model: we train a DNN in a \textit{single} multi-class classification problem (or multi-variate regression problem), keep all the layers except for the \textit{last} linear mapping and add one or \textit{more} extra layers to the remaining representation to adapt to new tasks.
% Another contribution of this paper is to first analyze the prediction function space beyond the linear mapping. Inspired by a lower bound construction for eluder dimension \citep{russo2013eluder,osband2014model}, 
%We found that the Eluder dimension \citep{russo2013eluder,osband2014model} that is used to measure sample complexity in Reinforcement Learning can be used to direct bound the performance on the target task. To be specific, we show that for any prediction function space $\mathcal{F}$, if its dual function space $\mathcal{F}^*$ has Eluder dimension $d$, then if the average error in source tasks can be bounded by $\epsilon$, then the error in target tasks can be upper bounded by $d \epsilon$ for some $d$ source tasks.

%\paragraph{Related works.}
%\cite{maurer2016benefit} assumes all the prediction function and the coefficients in source tasks should cover all the directions. \cite{tripuraneni2020theory} considers the general function class, where a diversity measure is proposed to guarantee the generalization. 

\section{Preliminaries}
We first introduce the mathematical setup of the problem studied in this paper along with the two-phase learning method that we will focus on.

\paragraph{Problem setup.} Let $\mathcal{X}$ denote the input space. We assume the same input distribution $P_X$  for all tasks, as covariate shift is not the focus of this work. In our representation learning setting, there exists a generic feature representation function $h^* \in \mathcal{H}:\mathcal{X} \mapsto \mathcal{Z}$ that is shared across different tasks, where $\mathcal{Z}$ is the feature space and $\mathcal{H}$ is the representation function space. Since we only consider the different prediction functions, each task, indexed by $t$, is defined by its prediction function $f_t^* \in \mathcal{F}_t:\mathcal{Z} \mapsto \mathcal{Y}_t$, where $\mathcal{F}_t$ is the prediction function space of task $t$ and $\mathcal{Y}_t$ is the corresponding output space. The observations $Y_t = f_t^* \circ h^* (X) + \epsilon$ are generated noisily with mean function $f_t^* \circ h^*$, where $X \sim P_{X}$ and $\epsilon$ is zero-mean noise that is independent of $X$.

%Formally, we denote a task $t$ by a tuple $\{\mathcal{X}, \mathcal{Z}, \mathcal{Y}_t, P_{X}, f^*_t \circ h^*\}$, where $\mathcal{X}$,$\mathcal{Z}$,$\mathcal{Y}$ are the feature space, representation space and response space respectively, $P_X$ is the distribution over $\mathcal{X}$, $h^* \in \mathcal{H}:\mathcal{X} \mapsto \mathcal{Z}$ is the task-independent representation function and $f^*_t \in \mathcal{F}_t:\mathcal{Z} \mapsto \mathcal{Y}$ is the task-specific prediction function. For each task $t$, the response variable is generated by $Y = f^*_t \circ h^*(X) + \epsilon \in \mathcal{Y}$, where $X \sim P_X$ and $\epsilon$ is some zero-mean noise. Note that for generality, we do not assume the same response space and covariate distribution across the tasks.

Our representation is learned on source tasks $\vect{f}^*_{so} \coloneqq (f_1^*, \dots, f_T^*) \in \mathcal{F}_{1} \times \dots \times \mathcal{F}_{T}$ for some positive integer $T$. We assume that all the prediction function spaces $\mathcal{F}_t = \mathcal{F}_{so}$ are the same over the source tasks. We denote the target task by $f^*_{ta} \in \mathcal{F}_{ta}$, where $\mathcal{F}_{ta}$ is the target prediction function space. Unlike the previous papers \citep{du2020few,tripuraneni2020theory,maurer2016benefit}, which all assume that the same prediction function space is used for all tasks, we generally allow for the possibility that $\mathcal{F}_{so} \neq \mathcal{F}_{ta}$.
%In other words, we are more interested in the discrepancy between source tasks and target task.

\paragraph{Learning algorithm.} 
We consider the same two-phase learning method as in \cite{tripuraneni2020theory}. In the first phase (the training phase), $\vect{n} = (n_1, \dots, n_T)$ samples from each task are available to learn a good representation. In the second phase (the test phase), we are presented $n_{ta}$ samples from the target task to learn its prediction function using the pretrained representation learned in the training phase.

We denote a dataset of size $n$ from task $f_t$ by $S^{n}_t = \{(x_{ti}, y_{ti})\}_{i = 1}^{n}$. We use empirical risk minimization (ERM) for both phase. In the training phase, we minimize average risks over $\{S_t^{n_t}\}_{t = 1}^{T}$:
$$
    \hat R(\vect{f}, {h} \mid \vect{f}^*_{so}) \coloneqq \frac{1}{\sum_t n_t}\sum_{t = 1}^T \sum_{i = 1}^{n_t} l_{so}(f_t \circ h(x_{ti}), y_{ti}),
$$
where $l_{so}: \mathcal{Y} \times \mathcal{Y} \mapsto \mathbb{R}$ is the loss function for the source tasks and $\vect{f} = (f_1, \dots, f_T) \in \mathcal{F}_{so}^{\otimes T}$. The estimates are given by $(\hat{\vect{f}}_{so}, \hat h) \in \argmin_{\vect{f}, h} \hat R(\vect{f}, h \mid \vect{f}^*_{so})$.
In the second phase, we obtain the dataset  $\{x_{ta, i}, y_{ta, i}\}_{i}^{n_{ta}}$ from the target task and our predictor $\hat f_{ta}$ is given by
$$
    \argmin_{f \in \mathcal{F}_{ta}} \hat R(f, \hat h \mid f_{ta}^*) \coloneqq \frac{1}{n_{ta}}\sum_{i = 1}^{n_{ta}} l_{ta}(f \circ \hat h(x_{ta, i}), y_{ta, i}),
$$
for some loss function $l_{ta}$ on the target task. We also use $R(\cdot, \cdot \mid \cdot)$ for the expectation of the above empirical risks. We denote the generalization error of certain estimates $f, h$ by $\mathcal{E}(f, h \mid \cdot) \coloneqq R(f, h \mid \cdot) -  \min_{f'\in\mathcal{F}, h' \in \mathcal{H}} R(f', h' \mid \cdot)$, where $\mathcal{F}$ can be either $\mathcal{F}_{so}^{\otimes T}$ or $\mathcal{F}_{ta}$ depending on the tasks. Our goal is to bound the generalization error of the target task. 

For simplicity, our results are presented under square loss functions. However, we show that our results can generalize to different loss functions in Appendix \ref{app:loss}. We also assume $n_1 = \dots = n_T = n_{so}$ for some positive integer $n_{so}$.

\subsection{Model complexity}
As this paper considers general function classes, our results will be presented in terms of the complexity measures of classes of functions. We follow the previous literature \citep{maurer2016benefit,tripuraneni2020theory} which uses Gaussian complexity. Note that we do not use the more common Rademacher complexity as the proofs require a decomposition theorem that only holds for Gaussian complexity. %The Gaussian complexity can be upper bounded by the 

For a generic vector-valued function class $\mathcal{Q}$ containing functions $q:\mathbb{R}^d \mapsto \mathbb{R}^r$ and $N$ data points, $X_N = (\vect{x}_1, \dots, \vect{x}_N)^T$, the empirical Gaussian complexity is defined\footnote{Note that the standard definition has a $1/N$ factor instead of $1/\sqrt{N}$. We use the variant so that $\hat{\mathfrak{G}}_N$ does not scale with $N$ in most of the cases we consider and only reflects the complexity of the class.} as
$$
    \hat{\mathfrak{G}}_{N}(\mathcal{Q})=\mathbb{E}_{\mathbf{g}}\left[\sup _{\mathbf{q} \in \mathcal{Q}} \frac{1}{\sqrt{N}} \sum_{i=1}^{N} g_{i}^T q(\vect{x}_{i})\right], \quad g_{i} \sim \mathcal{N}(0,I_r)\quad  i.i.d.
$$ %\ziping{Make this standard.}
The corresponding population Gaussian complexity is defined as $\mathfrak{G}_{N}(\mathcal{Q})=\mathbb{E}_{X_N}\left[\hat{\mathfrak{G}}_{N}(\mathcal{Q})\right]$, where the expectation is taken over the distribution of $X_N$.


%Let $\mathcal{F}(S_t^n) = \{f \in \mathcal{H}_t \circ \mathcal{G}: f(X_i) = f_t(X_i) \text{ for } i = 1, \dots, n\}$ be the subset of hypothesis space that is consistent with dataset $S_t^n$. Let $\mathcal{G}(S_t^n)$ and $\mathcal{H}(S_t^n)$ be the marginal space of $\mathcal{F}(S_t^n)$ on the representation and task-specific prediction function. For dataset $S_{\vect{s}}^{\vect{n}} \coloneqq (S_{s_1}^{n_{s_1}}, \dots S_{s_m}^{n_{s_m}})$ and $S_t^{n_t}$, our predictor on target task $t$ is any $f \in \mathcal{H}(S_t^{n_t}) \circ (\cap_{i = 1}^{m} \mathcal{G}(S_{s_i}^{n_{s_i}}))$.

% We evaluate a predictor $f$ by its error rate denoted by $\text{err}_t(f) \coloneqq \E_{X \sim P_{X_t}} \mathbbm{1}(f(X) \neq f_t(X))$.

%\begin{aspt}[Coverage on representation space] We say $S_{\vect{s}}^{\vect{n}}$ covers $S_t^{n_t}$ on representation space if $\cap_{i}\mathcal{G}(S_{s_i}^{n_{s_i}}) \subset \mathcal{G}(S_t^{n_t})$. Furthermore, we say tasks $s_1, \dots s_m$ have coverage $n_{\vect{s}, t}(\vect{n}, \delta) \in \mathbbm{N}$ if random sampled datasets $S_{\vect{s}}^{\vect{n}}$ covers $S_t^{n_t(n_1, \dots, n_m, \delta)}$ with a probability at least $1-\delta$, where $n_{\vect{s}, t}$ maps $\mathbbm{N}^m \times \mathbbm{R}$ to $\mathbbm{N}$. \end{aspt}



\subsection{Diversity}
Source tasks have to be diverse enough, to guarantee that the representation learned from source tasks can be generalized to any target task in $\mathcal{F}_{ta}$. %For example, consider the representation space $\mathcal{Z} \subset \mathbb{R}^d$ and $\mathcal{F}_{so} = \mathcal{F}_{ta} = \{w^Tz: w \in \mathbb{R}^d, \|w\|_2 \leq 1\}$. Generally speaking, a single source task with $w = (1, 0, \dots, 0)$ can not help learn target task with $w = (0, 1, 0, \dots, 0)$ as the two vectors are orthogonal. 
To measure when transfer can happen, we introduce the following two definitions, namely that of \textit{transferability} and \textit{diversity}.

\begin{defn}
\label{defn:transferable}
For some $\nu, \mu > 0$, we say the source tasks $f_1^*, \dots, f_T^* \in \mathcal{F}_{so}$ are $(\nu, \mu)$-transferable to task $f_{ta}^*$ if 
$$
    \sup_{h \in \mathcal{H}} \frac{\inf_{f \in \mathcal{F}_{ta}}\mathcal{E}(f, h \mid f_{ta}^*)}{\inf_{\vect{f} \in \mathcal{F}_{so}^{\otimes T}}\mathcal{E}(\vect{f}, h \mid \vect{f}^*_{so}) + \mu / \nu} \leq \nu.
$$
Furthermore, we say they are $(\nu, \mu)$-diverse over $\mathcal{F}_{ta}$ if above ratio is bounded for any true target prediction functions $f_{ta}^* \in \mathcal{F}_{ta}$, i.e.
$$
        \sup_{f_{ta}^* \in \mathcal{F}_{ta}}\sup_{h \in \mathcal{H}} \frac{\inf_{f \in \mathcal{F}_{ta}}\mathcal{E}(f, h \mid f_{ta}^*)}{\inf_{\vect{f} \in \mathcal{F}_{so}^{\otimes T}}\mathcal{E}(\vect{f}, h \mid \vect{f}^*_{so}) + \mu / \nu} \leq \nu.
$$
\end{defn}

%Note that as each task corresponds to a prediction function, we will also say a set of functions is $(\nu, \mu)$-transferable to a function $f_{ta}^*$.
When it is clear from the context, we denote $\mathcal{E}(f, h \mid f_{ta}^*)$ and $\mathcal{E}(\vect{f}, h \mid \vect{f}_{so}^*)$ by $\mathcal{E}_{ta}(f, h)$ and $\mathcal{E}_{so}(\vect{f}, h)$, respectively. We will call $\nu$ the transfer component and $\mu$, the bias introduced by transfer. 
The definition of transferable links the generalization error between source tasks and the target task as shown in Theorem \ref{thm:approx_error1}. The proof can be found in Appendix \ref{app:approx_error1}.
\begin{thm}
\label{thm:approx_error1}
If source tasks $f_1^*, \dots, f_T^*$ are $(\nu, \mu)$-diverse over $\mathcal{F}_{ta}$, then for any $f_{ta}^* \in \mathcal{F}_{ta}$, we have
$$
    \mathcal{E}_{ta}(\hat f_{ta}, \hat h) \leq \nu \mathcal{E}_{so}({\hat{\vect{f}}_{so}}, \hat h) + \mu +  \frac{\sqrt{2 \pi} \hat{\mathfrak{G}}_{n_{t a}}\left(\mathcal{F}_{t a} \circ \hat{h}\right)}{\sqrt{n_{t a}}}+\sqrt{\frac{9 \ln (2 / \delta)}{2 n_{t a}}}.
$$
%where $\hat{\vect{f}}_{so} \in \argmin_{\vect{f} \in \mathcal{F}_{so}^{\otimes T}} \min_{h} \hat R_{so}(\vect{f}, h)$.
\end{thm}

The first term in Theorem \ref{thm:approx_error1} can be upper bounded using the standard excess error bound of Gaussian complexity. The benefit of representation learning is due to the decrease in the third term from $\hat{\mathfrak{G}}_{n_{t a}}(\mathcal{F}_{t a} \circ \mathcal{H})/\sqrt{n_{ta}}$ without representation learning to $\hat{\mathfrak{G}}_{n_{t a}}(\mathcal{F}_{t a} \circ \hat{h})/\sqrt{n_{ta}}$ in our case. For the problem with complicated representations, the former term can be extremely larger than the later one.

In the rest of the paper, we discuss when we can bound $(\nu, \mu)$, for nonlinear and nonidentical $\mathcal{F}_{so}$ and $\mathcal{F}_{ta}$.
% In the rest of the paper, we will mainly discuss when the diversity can be achieved for different $\mathcal{F}_{so}$'s and $\mathcal{F}_{ta}$'s. In section \ref{sec:negative_res}, we discuss a negative case where no representation learning benefit can be achieved. In section \ref{sec:sour_repre}, we introduce a special case where diversity can be easily bounded when source tasks are diverse over its own space $\mathcal{F}_{so}$ and the target task is more complex than the source tasks in the way that $\mathcal{F}_{ta} = \mathcal{F}'_{ta} \circ (\mathcal{F}_{so}^{\otimes m})$. We further discuss the applications to deep neural network prediction functions. In section \ref{sec:div_general}, we consider a sufficient condition of source tasks being diverse over its own space $\mathcal{F}_{so}$ by making an interesting connection to Eluder dimension. In section \ref{sec:multiclass}, we show that a single multiclass classification task can be diverse. In the last section, we use four experiments to verify the theoretical results in section \ref{sec:sour_repre} and \ref{sec:div_general}.

\iffalse
\section{Bounding approximation error}


\subsection{Generalization error decomposition}
Equation (\ref{equ:tar_ge}) bounds the total generalization with two terms, the approximation error of using $\hat g$ and the generalization error over a smaller class $\mathcal{H}_t \circ \hat g$. As $\hat{\mathfrak{G}}_{n}(\mathcal{H}_t \circ \hat g)$ is significantly smaller than $\hat{\mathfrak{G}}_{n}(\mathcal{H}_t \circ \mathcal{G})$, the desired representation learning improves the risk bound if approximation error scales with $1/\sum_t n_t$.

%We first look at the case, where only one source task is available. 
To control the approximation error, we introduce the following similarity measure. Note that this is a general form of the transfer exponent assumption in \cite{hanneke2020no}, which assumes $\mathcal{E}_{so}(h) \leq C_{\rho}\mathcal{E}_{ta}^{1/\rho}(h)$ for all $h$. In this paper, we focus on the $C_{\rho}$ coefficient and generalize the assumption to the representation learning setting, which assumes that for any representation $g$, the best prediction function has a similar exponent. \cite{tripuraneni2020theory} consider the same measure, while their definition requires the same constants holding for all the target tasks with different prediction functions in $\mathcal{H}_{ta}$.


Intuitively, when $\mathcal{S}$ is $(\nu, \mu)$-transferable to $ta$, any representation that yields a low risk on $\mathcal{S}$ should also have a low approximation error on the target task with respective to a difference of $\mu/\nu$, which is formalized in Proposition \ref{prop:approx_error1}.

\begin{thm}
\ziping{We require the composition is also bounded by $B$.}
\label{thm:2}
If $\mathcal{S}$ is $(\nu, \mu)$-transferable to task $ta$, then 
$$
\mathcal{E}_{t a}(\hat{h}_{t a} \circ \hat{g}) = \tilde{\mathcal{O}}\left(\frac{\nu \hat{\mathfrak{G}}_{{\sum_{s} n_s}}(\mathcal{H}_{so}^{\otimes S} \circ \mathcal{G})}{\sqrt{\sum_s n_{s}}} + \frac{ \hat{\mathfrak{G}}_{n_{ta}}(\mathcal{H}_{ta}\circ \hat g)}{\sqrt{n_{ta}}} + \mu \right)
$$
\end{thm}

\begin{proof}
It remains to bound $\mathcal{E}_{so}(\hat{\vect{h}}_{so}, \hat g)$. Theorem 1 in \cite{tripuraneni2020theory} show that with a probability at least $1-\delta$,
$$
    \mathcal{E}_{so}(\hat{\vect{h}}_{so}, \hat g) \leq 16 L \mathfrak{G}_{\sum_{s}n_s}\left(\mathcal{H}_{so}^{\otimes S} \circ \mathcal{G}\right)+8 B \sqrt{\frac{\log (2 / \delta)}{\sum_s n_s}},
$$
where $L$ is the Lipschitz constant of loss function $l_{so}$ and $l_{so}$ is $B$-bounded. Combined with (\ref{equ:tar_ge}), the theorem follows.

\end{proof}

Note that \cite{tripuraneni2020theory} shows that under linear prediction function with neural network representations, the diversity assumption is satisfied if the coefficients of the linear functions covers all the directions. However, to answer the questions we proposed in the introduction section, we consider the following special structures, where we do not need multiple source tasks to have assumption 1 hold.
\fi

==> Representation%20Learning%20(Version%2012650)/wrong_proof1.tex <==
Now we consider a more general case. Previously, we assume that $h_t \circ g$. Now we consider a more general case, where the target task use the outputs of several different tasks in source task set as representation. Formally, we define $\mathcal{H}_{ta} = \mathcal{H}'_{ta} \circ \mathcal{M}$ and $\mathcal{H}_{so} = \mathcal{H}'_{so} \circ \mathcal{M}$ for some shared class $\mathcal{M}:\mathcal{Z} \mapsto \mathbbm{R}^d$ and task-specific class $\mathcal{H}'_{ta}$ and $\mathcal{H}'_{so}$ from $\mathbbm{R}^d$ to $\mathcal{Y}_{so}$ and $\mathcal{Y}_{ta}$, respectively. Note that if $\mathcal{H}'_{so} \subset \mathcal{H}'_{ta}$, we have $\mathcal{H}_{so} \subset \mathcal{H}_{ta}$ and target task is strictly harder than the source task.


We first introduce the diversity definition in \cite{tripuraneni2020theory}. 
\begin{defn}[\cite{tripuraneni2020theory}]
Following Definition \ref{defn:transferable}, we say a task set $\mathcal{S}$ is $(\nu, \mu)$-diverse over a function class $\mathcal{H}$ with loss function $l$, if it is $(\nu, \mu)$-transferable to any task with prediction function in $\mathcal{H}$ and loss function $l$.
\end{defn}

\begin{aspt} 
\label{aspt:2}
Assume Assumption \ref{aspt:cont_tar} (a), (b), (c) hold, and we further assume
\begin{enumerate}[label=(\alph*)]
    \item There exists $k$ functions $h'_{1}, \dots, h'_{k} \in \mathcal{H}'_{so}$ such that $A(x)A(y)^T \succ c_4 I_d$ with $A(\cdot) = (\nabla h_{1}(\cdot), \dots, \nabla h_{k}(\cdot))$ for any $x, y \in \mathbbm{R}^d$.
    \item Any $h'_{ta} \in \mathcal{H}'_{ta}$ is $c_5$-Lipschitz with respect to $l_2$ distance.
\end{enumerate}
\end{aspt}

\begin{thm}
\label{thm:general_case}
If task set $\mathcal{S}$ is $(\nu, \mu)$-diverse over its own class $\mathcal{H}_{so}$, Assumption \ref{aspt:2} holds, we have 
$$
    \mathcal{E}_{ta}\left(\hat{h}_{ta}, \hat{g}\right)=\tilde{\mathcal{O}}\left( \frac{c_2c_5d \nu}{c_4c_1}\left(\frac{\hat{\mathfrak{G}}_{\sum_s n_{s}}\left( \mathcal{G}\right)}{\sqrt{\sum_s n_{s}}} +
    \frac{\hat{\mathfrak{G}}_{\bar{n}_{so}}\left(     \mathcal{H}_{so}\right)}{\sqrt{\bar{n}_{so}}} + \mu\right)
    + \frac{\hat{\mathfrak{G}}_{n_{t a}}\left(\mathcal{H}_{ta} \circ \hat{g}\right)}{\sqrt{n_{t a}}}
    \right).
$$
\end{thm}

\begin{proof}
We first show that $\mathcal{S}$ is also $(\nu, \mu)$-diverse over $\mathcal{M}$. To show that, for any $g \in \mathcal{G}$, we lower bound the following term with $Y = h'^*_{so}\circ m^*(X) + \epsilon$,
\begin{align*}
    &\quad \sup_{h'^*_{so}\circ m^*}  \E_{X, Y} l_{so}(h'^*_{so}\circ m^* \circ g^*(X), Y) - l_{so}(h'^*_{so}\circ m^* \circ g(X), Y)\\
    &\quad\quad \text{(using Assumption \ref{aspt:cont_tar} (a))}\\
    &\geq c_1 \sup_{h_{s o}^{\prime *} \circ m^{*}} \E_X\|h_{so}^{\prime *} \circ m^{*} \circ g^*(X) - h_{so}^{\prime *} \circ m^{*} \circ g(X)\|_2^2 \\
    &\geq \frac{c_1}{k} \sup_{m^*} \E_X \sum_{i=1}^k \|h_i' \circ m^* \circ g^*(X) - h_i' \circ m^* \circ g(X) \|_2^2 \\
    &\geq \frac{c_1}{k} \sup_{m^*} \E_X  \|\sum_{i=1}^k (h_i' \circ m^* \circ g^*(X) - h_i' \circ m^* \circ g(X))\|_2^2  \numberthis \label{equ:thm4_prf1}
\end{align*}

Now for any $x$, we denote $m^* \circ g^*(x)$ and $m^* \circ g(x)$ by $a_1$ and $a_2$, respectively. By calculus,
\begin{align*}
    &\quad  h_i'(a_1) - h_i'(a_2) 
    = (a_1 - a_2)^T(\int_{0}^1 \nabla h_i'(ta_1 + (1-t)a_2) dt) 
\end{align*}


Denote $\nabla h_i'(ta_1 + (1-t)a_2)$ by $A_i(t)$ and $\vect{A}(t) = \left(A_{1}(t), \ldots, A_{k}(t)\right)$. Then by Assumption \ref{aspt:2} (a),
$$
(\int_{0}^1 \vect{A}(t) dt)(\int_{0}^1 \vect{A}(t) dt)^T \succ c_4 I
$$
Thus, we have
$$
    \sum_{i=1}^k\| h_i'(a_1) - h_i'(a_2) \|_2^2 = (a_1 - a_2)^T \left((\int_{0}^1 \vect{A}(t) dt)(\int_{0}^1 \vect{A}(t) dt)^T\right)(a_1 - a_2) \geq c_4\|a_1 - a_2\|_2^2.
$$
Plug this into (\ref{equ:thm4_prf1}), we get 
$$
    \sup_{h'^*_{so}\circ m^*}  \E_{X, Y} l_{so}(h'^*_{so}\circ m^* \circ g^*(X), Y) - l_{so}(h'^*_{so}\circ m^* \circ g(X), Y) \geq \frac{c_1c_4}{k} \sup_{m^*}\E_X\|m^*\circ g^*(X) - m^*\circ g(X)\|_2^2,
$$
which shows that the source tasks set $\mathcal{S}$ is also $(\frac{k\nu}{c_1c_4}, \frac{k\mu}{c_1c_4})$-diverse over $\mathcal{M}$ with $L_2$ loss.

Now that 
\begin{align*}
    \mathcal{E}_{ta}(h'^*_{ta}\circ m_{ta}^*, g) 
    &\leq \frac{c_2c_3}{2} \E_X\|m^*_{ta}\circ g(X) - m^*_{ta}g^*(X)\|_2^2\\
    &\leq \frac{c_2c_3}{2} \sup_{m^*}  \mathbb{E}_{X} \| m^{*} \circ g^{*}(X)-m^{*} \circ g(X)\|_2^2\\
    &\leq \frac{k c_2c_3}{c_1c_4} (\nu\mathcal{E}_{so}(\vect{h}^*_{so}, \hat g) + \mu)
\end{align*}
%where $h'^*_{so}$ is taken over $\mathcal{H}_{so}'$ and $m^*$ is taken over $\mathcal{M}$.

%\sup_{m^*} \E_{X}\|m^*\circ g^*(X) - m^*\circ g(X)\|_2^2, \ziping{define $\mathcal{E}_{f}$ here}



\end{proof}

==> wrong_proof1.tex <==
Now we consider a more general case. Previously, we assume that $h_t \circ g$. Now we consider a more general case, where the target task use the outputs of several different tasks in source task set as representation. Formally, we define $\mathcal{H}_{ta} = \mathcal{H}'_{ta} \circ \mathcal{M}$ and $\mathcal{H}_{so} = \mathcal{H}'_{so} \circ \mathcal{M}$ for some shared class $\mathcal{M}:\mathcal{Z} \mapsto \mathbbm{R}^d$ and task-specific class $\mathcal{H}'_{ta}$ and $\mathcal{H}'_{so}$ from $\mathbbm{R}^d$ to $\mathcal{Y}_{so}$ and $\mathcal{Y}_{ta}$, respectively. Note that if $\mathcal{H}'_{so} \subset \mathcal{H}'_{ta}$, we have $\mathcal{H}_{so} \subset \mathcal{H}_{ta}$ and target task is strictly harder than the source task.


We first introduce the diversity definition in \cite{tripuraneni2020theory}. 
\begin{defn}[\cite{tripuraneni2020theory}]
Following Definition \ref{defn:transferable}, we say a task set $\mathcal{S}$ is $(\nu, \mu)$-diverse over a function class $\mathcal{H}$ with loss function $l$, if it is $(\nu, \mu)$-transferable to any task with prediction function in $\mathcal{H}$ and loss function $l$.
\end{defn}

\begin{aspt} 
\label{aspt:2}
Assume Assumption \ref{aspt:cont_tar} (a), (b), (c) hold, and we further assume
\begin{enumerate}[label=(\alph*)]
    \item There exists $k$ functions $h'_{1}, \dots, h'_{k} \in \mathcal{H}'_{so}$ such that $A(x)A(y)^T \succ c_4 I_d$ with $A(\cdot) = (\nabla h_{1}(\cdot), \dots, \nabla h_{k}(\cdot))$ for any $x, y \in \mathbbm{R}^d$.
    \item Any $h'_{ta} \in \mathcal{H}'_{ta}$ is $c_5$-Lipschitz with respect to $l_2$ distance.
\end{enumerate}
\end{aspt}

\begin{thm}
\label{thm:general_case}
If task set $\mathcal{S}$ is $(\nu, \mu)$-diverse over its own class $\mathcal{H}_{so}$, Assumption \ref{aspt:2} holds, we have 
$$
    \mathcal{E}_{ta}\left(\hat{h}_{ta}, \hat{g}\right)=\tilde{\mathcal{O}}\left( \frac{c_2c_5d \nu}{c_4c_1}\left(\frac{\hat{\mathfrak{G}}_{\sum_s n_{s}}\left( \mathcal{G}\right)}{\sqrt{\sum_s n_{s}}} +
    \frac{\hat{\mathfrak{G}}_{\bar{n}_{so}}\left(     \mathcal{H}_{so}\right)}{\sqrt{\bar{n}_{so}}} + \mu\right)
    + \frac{\hat{\mathfrak{G}}_{n_{t a}}\left(\mathcal{H}_{ta} \circ \hat{g}\right)}{\sqrt{n_{t a}}}
    \right).
$$
\end{thm}

\begin{proof}
We first show that $\mathcal{S}$ is also $(\nu, \mu)$-diverse over $\mathcal{M}$. To show that, for any $g \in \mathcal{G}$, we lower bound the following term with $Y = h'^*_{so}\circ m^*(X) + \epsilon$,
\begin{align*}
    &\quad \sup_{h'^*_{so}\circ m^*}  \E_{X, Y} l_{so}(h'^*_{so}\circ m^* \circ g^*(X), Y) - l_{so}(h'^*_{so}\circ m^* \circ g(X), Y)\\
    &\quad\quad \text{(using Assumption \ref{aspt:cont_tar} (a))}\\
    &\geq c_1 \sup_{h_{s o}^{\prime *} \circ m^{*}} \E_X\|h_{so}^{\prime *} \circ m^{*} \circ g^*(X) - h_{so}^{\prime *} \circ m^{*} \circ g(X)\|_2^2 \\
    &\geq \frac{c_1}{k} \sup_{m^*} \E_X \sum_{i=1}^k \|h_i' \circ m^* \circ g^*(X) - h_i' \circ m^* \circ g(X) \|_2^2 \\
    &\geq \frac{c_1}{k} \sup_{m^*} \E_X  \|\sum_{i=1}^k (h_i' \circ m^* \circ g^*(X) - h_i' \circ m^* \circ g(X))\|_2^2  \numberthis \label{equ:thm4_prf1}
\end{align*}

Now for any $x$, we denote $m^* \circ g^*(x)$ and $m^* \circ g(x)$ by $a_1$ and $a_2$, respectively. By calculus,
\begin{align*}
    &\quad  h_i'(a_1) - h_i'(a_2) 
    = (a_1 - a_2)^T(\int_{0}^1 \nabla h_i'(ta_1 + (1-t)a_2) dt) 
\end{align*}


Denote $\nabla h_i'(ta_1 + (1-t)a_2)$ by $A_i(t)$ and $\vect{A}(t) = \left(A_{1}(t), \ldots, A_{k}(t)\right)$. Then by Assumption \ref{aspt:2} (a),
$$
(\int_{0}^1 \vect{A}(t) dt)(\int_{0}^1 \vect{A}(t) dt)^T \succ c_4 I
$$
Thus, we have
$$
    \sum_{i=1}^k\| h_i'(a_1) - h_i'(a_2) \|_2^2 = (a_1 - a_2)^T \left((\int_{0}^1 \vect{A}(t) dt)(\int_{0}^1 \vect{A}(t) dt)^T\right)(a_1 - a_2) \geq c_4\|a_1 - a_2\|_2^2.
$$
Plug this into (\ref{equ:thm4_prf1}), we get 
$$
    \sup_{h'^*_{so}\circ m^*}  \E_{X, Y} l_{so}(h'^*_{so}\circ m^* \circ g^*(X), Y) - l_{so}(h'^*_{so}\circ m^* \circ g(X), Y) \geq \frac{c_1c_4}{k} \sup_{m^*}\E_X\|m^*\circ g^*(X) - m^*\circ g(X)\|_2^2,
$$
which shows that the source tasks set $\mathcal{S}$ is also $(\frac{k\nu}{c_1c_4}, \frac{k\mu}{c_1c_4})$-diverse over $\mathcal{M}$ with $L_2$ loss.

Now that 
\begin{align*}
    \mathcal{E}_{ta}(h'^*_{ta}\circ m_{ta}^*, g) 
    &\leq \frac{c_2c_3}{2} \E_X\|m^*_{ta}\circ g(X) - m^*_{ta}g^*(X)\|_2^2\\
    &\leq \frac{c_2c_3}{2} \sup_{m^*}  \mathbb{E}_{X} \| m^{*} \circ g^{*}(X)-m^{*} \circ g(X)\|_2^2\\
    &\leq \frac{k c_2c_3}{c_1c_4} (\nu\mathcal{E}_{so}(\vect{h}^*_{so}, \hat g) + \mu)
\end{align*}
%where $h'^*_{so}$ is taken over $\mathcal{H}_{so}'$ and $m^*$ is taken over $\mathcal{M}$.

%\sup_{m^*} \E_{X}\|m^*\circ g^*(X) - m^*\circ g(X)\|_2^2, \ziping{define $\mathcal{E}_{f}$ here}



\end{proof}
